High-Performance Statistical Computing in the Computing Environments of the 2020s

Technological advances in the past decade, hardware and software alike, have made access to high-performance computing (HPC) easier than ever. We review these advances from a statistical computing perspective. Cloud computing makes access to supercomputers affordable. Deep learning software libraries make programming statistical algorithms easy and enable users to write code once and run it anywhere -- from a laptop to a workstation with multiple graphics processing units (GPUs) or a supercomputer in a cloud. Highlighting how these developments benefit statisticians, we review recent optimization algorithms that are useful for high-dimensional models and can harness the power of HPC. Code snippets are provided to demonstrate the ease of programming. We also provide an easy-to-use distributed matrix data structure suitable for HPC. Employing this data structure, we illustrate various statistical applications including large-scale positron emission tomography and $\ell_1$-regularized Cox regression. Our examples easily scale up to an 8-GPU workstation and a 720-CPU-core cluster in a cloud. As a case in point, we analyze the onset of type-2 diabetes from the UK Biobank with 200,000 subjects and about 500,000 single nucleotide polymorphisms using the HPC $\ell_1$-regularized Cox regression. Fitting this half-million-variate model takes less than 45 minutes and reconfirms known associations. To our knowledge, this is the first demonstration of the feasibility of penalized regression of survival outcomes at this scale.

==> sections/00_abstract.tex <==
\iffalse
Recent development made access to high-performance computing easier than ever for statisticians.
Hardware with high maintenance costs for statisticians is now accessible through clouds. 
Programming models are unified for computation on various hardware. 
Scalable algorithms that are useful in a distributed-memory setting are developed. 
In this work, we review advances in hardware accessibility, programming tools, and algorithms for harnessing the computing power of multi-machine or multi-GPU settings. 
Examples on several statistical computing tasks, including nonnegative matrix factorization,  positron emission tomography, multidimensional scaling, and $\ell_1$-regularized Cox regression are provided. 
We scale up our experiments over an 8-GPU local machine for the multi-GPU setting and over 20 virtual CPU machines or 720 CPU cores for the virtual cluster setting on the Amazon Web Services cloud.
We show Code snippets are provided to ease the use of computational statisticians.
\fi

==> sections/BA_technical.tex <==
\section{Technical importance of unified interfaces for various HPC enviornments}\label{sec:why}
The feature of unified interfaces for various HPC environments is 
supported through operator overloading or polymorphism in modern programming languages,
but achieving this seamlessly with a single library, along with multi-device support, is remarkable. 
This is partially because of injection of capital in pursuit of commercial promises of deep learning (TensorFlow is being developed by Google, and PyTorch by Facebook).
%
There are other deep learning software libraries with similar HPC supports: 
Apache MxNet \citep{chen2015mxnet} supports multi-node computation via Horovod; multi-GPU computing is also supported at the interface level.
Microsoft Cognitive Toolkit \citep[CNTK,][]{seide2016cntk} supports parallel stochastic gradient algorithms through MPI.
